GeoSim: Realistic Video Simulation via Geometry-Aware Composition for Self-Driving

Scalable sensor simulation is an important yet challenging open problem for safety-critical domains such as self-driving. Current works in image simulation either fail to be photorealistic or do not model the 3D environment and the dynamic objects within, losing high-level control and physical realism. In this paper, we present GeoSim, a geometry-aware image composition process which synthesizes novel urban driving scenarios by augmenting existing images with dynamic objects extracted from other scenes and rendered at novel poses. Towards this goal, we first build a diverse bank of 3D objects with both realistic geometry and appearance from sensor data. During simulation, we perform a novel geometry-aware simulation-by-composition procedure which 1) proposes plausible and realistic object placements into a given scene, 2) render novel views of dynamic objects from the asset bank, and 3) composes and blends the rendered image segments. The resulting synthetic images are realistic, traffic-aware, and geometrically consistent, allowing our approach to scale to complex use cases. We demonstrate two such important applications: long-range realistic video simulation across multiple camera sensors, and synthetic data generation for data augmentation on downstream segmentation tasks. Please check https://tmux.top/publication/geosim/ for high-resolution video results.

==> fig_argo.tex <==
\begin{figure*}[t]
\centering
\scalebox{1}{
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ccccc}
\includegraphics[width=0.24\linewidth]{figs/argoverse_res/2bc31_result.png}
& \includegraphics[width=0.24\linewidth]{figs/argoverse_res/31_result.png}
& \includegraphics[width=0.24\linewidth]{figs/argoverse_res/41_result.png}
& \includegraphics[width=0.24\linewidth]{figs/argoverse_res/49d31_result.png}\\
\includegraphics[width=0.24\linewidth]{figs/argoverse_res/49d_41_result.png}
& \includegraphics[width=0.24\linewidth]{figs/argoverse_res/49d_71_result.png}
& \includegraphics[width=0.24\linewidth]{figs/argoverse_res/10b_21_result.png}
& \includegraphics[width=0.24\linewidth]{figs/argoverse_res/9573_41_result.png}\\
\end{tabular}}

\caption{\textbf{Qualitative Results in Argoverse.} 
}
\label{fig:argo_qual}
\end{figure*}


==> fig_results.tex <==
\begin{figure}[!htbp]
\vspace{-0.3cm}
\centerline{ 
\begin{tabular}{cccc}
	Before & After & {\tt pix2pixHD} \cite{wang_high-resolution_2017} & {\tt Copy \& Paste} \cite{portenier_smart_2019} \\
	\includegraphics[width=0.25\textwidth]{./figs/results/000befec-5265-49b0-cf02-3db58ebd95e8_200_12_bg_img.png.jpg} &
	\includegraphics[width=0.25\textwidth]{./figs/results/000befec-5265-49b0-cf02-3db58ebd95e8_200_12_synthesized.png.jpg}
	& \includegraphics[width=0.25\textwidth]{./figs/results/000befec-5265-49b0-cf02-3db58ebd95e8_000_12_sem.png.jpg}  %
	& \includegraphics[width=0.25\textwidth]{./figs/results/000befec-5265-49b0-cf02-3db58ebd95e8_000_12_sem.png.jpg} \\ %
	\includegraphics[width=0.25\textwidth]{./figs/results/0530e56b-eac8-404b-fd55-8490a158da97_200_12_bg_img.png.jpg} & %
	\includegraphics[width=0.25\textwidth]{./figs/results/0530e56b-eac8-404b-fd55-8490a158da97_200_12_synthesized.png.jpg}
	& \includegraphics[width=0.25\textwidth]{./figs/results/000befec-5265-49b0-cf02-3db58ebd95e8_000_12_sem.png.jpg}  %
	& \includegraphics[width=0.25\textwidth]{./figs/results/000befec-5265-49b0-cf02-3db58ebd95e8_000_12_sem.png.jpg} \\ %
	\includegraphics[width=0.25\textwidth]{./figs/results/05acd26d-48d7-4492-c7c1-c06b54573b7e_100_12_bg_img.png.jpg} &
	\includegraphics[width=0.25\textwidth]{./figs/results/05acd26d-48d7-4492-c7c1-c06b54573b7e_100_12_synthesized.png.jpg}
	& \includegraphics[width=0.25\textwidth]{./figs/results/000befec-5265-49b0-cf02-3db58ebd95e8_000_12_sem.png.jpg}  %
	& \includegraphics[width=0.25\textwidth]{./figs/results/000befec-5265-49b0-cf02-3db58ebd95e8_000_12_sem.png.jpg} \\ %
	\includegraphics[width=0.25\textwidth]{./figs/results/00d0ebbc-592c-431d-f3e9-c5b13131e946_000_12_bg_img.png.jpg} &
	\includegraphics[width=0.25\textwidth]{./figs/results/00d0ebbc-592c-431d-f3e9-c5b13131e946_000_12_synthesized.png.jpg}
	& \includegraphics[width=0.25\textwidth]{./figs/results/000befec-5265-49b0-cf02-3db58ebd95e8_000_12_sem.png.jpg}  %
	& \includegraphics[width=0.25\textwidth]{./figs/results/000befec-5265-49b0-cf02-3db58ebd95e8_000_12_sem.png.jpg} \\  %
	\includegraphics[width=0.25\textwidth]{./figs/results/022d075e-6dd7-481f-ff28-1c55705deaba_100_12_bg_img.png.jpg} &
	\includegraphics[width=0.25\textwidth]{./figs/results/022d075e-6dd7-481f-ff28-1c55705deaba_100_12_synthesized.png.jpg}
	& \includegraphics[width=0.25\textwidth]{./figs/results/000befec-5265-49b0-cf02-3db58ebd95e8_000_12_sem.png.jpg}  %
	& \includegraphics[width=0.25\textwidth]{./figs/results/000befec-5265-49b0-cf02-3db58ebd95e8_000_12_sem.png.jpg} \\ %
\end{tabular}}
\caption{Left: initial background scene. Center: scene after dynamic object placement and re-rendering. Right two columns: {\tt pix2pixHD} \cite{wang_high-resolution_2017} conditioned on the same semantic layout as the center image and {\tt Copy \& Paste} \cite{portenier_smart_2019} conditioned only on the background. Further examples are available in the supplementary materials. [TODO replace placeholder images for comparisons]}
\label{figure:samples}
\end{figure} 


